Machine Learning on Volatile Instances

Due to the massive size of the neural network models and training datasets used in machine learning today, it is imperative to distribute stochastic gradient descent (SGD) by splitting up tasks such as gradient evaluation across multiple worker nodes. However, running distributed SGD can be prohibitively expensive because it may require specialized computing resources such as GPUs for extended periods of time. We propose cost-effective strategies to exploit volatile cloud instances that are cheaper than standard instances, but may be interrupted by higher priority workloads. To the best of our knowledge, this work is the first to quantify how variations in the number of active worker nodes (as a result of preemption) affects SGD convergence and the time to train the model. By understanding these trade-offs between preemption probability of the instances, accuracy, and training time, we are able to derive practical strategies for configuring distributed SGD jobs on volatile instances such as Amazon EC2 spot instances and other preemptible cloud instances. Experimental results show that our strategies achieve good training performance at substantially lower cost.

==> 1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\GJ{In the paragraph below, I suggest adding something like this: Stochastic gradient descent is at the backbone of most state-of-the-art machine learning problems. Due to the massive size neural network models and training datasets used today, it is imperative to distribute the task of computing gradients across multiple computing nodes. Currently, even such distributed machine learning jobs require high-performance computing infrastructure such as GPUs. Renting such machines as on-demand instances from services like Amazon EC2 can be prohibitively expensive because distributed training jobs can take hours or even days to complete.}

\carlee{I agree with Gauri's suggested outline. Then we can say that in some cases, we can save money by running jobs on other types of machines or instances. Such machines generally promise lower cost at the expense of lower reliability, which leads to performance tradeoffs. Spot instances are a well known example of this, and then we introduce other possible use cases.}

Large-scale machine learning training jobs usually require large amounts of computing resources, \eg, GPUs, which are expensive; these algorithms generally also have long runtimes due to the amount of data that they need to process. Such jobs are generally run in cloud servers in order to avoid the maintenance and investment costs associated with purchasing excessive numbers of servers. Today's machine learning jobs can be decentralized, where multiple distributed workers perform the training algorithm in parallel, each of which processes a subset of the dataset. The training algorithm that we focus on in this work, is the widely adopted distributed Stochastic Gradient Descent (SGD) algorithm, where multiple workers solve for an unconstrained optimization problem by communicating with a central parameter server and iteratively updating the gradients of the objective function using randomly chosen samples in the dataset.

Even in distributed settings, since a large amount of resource-time is required, it can be expensive if running on machines that adopt the pay-as-you-go pricing policy, \eg, on-demand instances on Amazon EC2. To save cost, they can consider Amazon EC2 Spot instances. The price of Spot instances are adjusted by Amazon EC2 based on long-term trends in supply and demand for Spot instance capacity. 
By setting the bid price as the maximum price that the user can accept, the user' job will only be running when the Spot price is below the bid price.
It is also shown that users can enjoy a discount up to $90\%$-off compared with using on-demand instances.
Therefore, running jobs on Spot instances can save cost especially for long lived jobs if tolerable to interruptions.

\carlee{add a paragraph on distributed clouds and wireless devices: other reasons that the workers may be unreliable. Maybe if the devices share a network connection, they will have correlated failure rates due to unstable connectivity?}

\subsection{Use Cases}

Amazon allows two types of job requests, one-time and persistent. A job with a one-time request will be terminated once the Spot price exceeds the user's bid price; a job with a persistent request will be interrupted due to the Spot price being high and resumed once the Spot price falls below the bid price again. Machine learning jobs can be persistent. In \cite{persistent}, the author shows several approaches to circumvent the weaknesses of Spot instances for supporting machine learning jobs. In this work, we assume a persistent request of each job. \GJ{It seems a bit early to talk about persistent and one-time requests. Maybe we can shift this to the system model/problem formulation section and keep the introduction at a high-level?}

In this work, we aim to design optimal bids such that the expected cost is minimized while a few constraints of each job is satisfied. \carlee{rewrite this--goal is to understand accuracy vs. latency tradeoffs when devices are not reliable. Optimal bidding falls out of this characterization.} We assume each worker is deployed on a Spot instance. 

\subsection{Challenges and Contributions}

\GJ{This section is too detailed in my opinion. The high-level problem and its interesting dimensions are not clear yet. Under challenges you can say that choice of the bid price the overall training runtime since instances can get interrupted. Bidding higher can allow us to retain many instances, but the marginal benefit of more instances in improving convergence speed reduces. Thus, it is non-trivial to choose the right bid price. Our contribution is to analyze the effect of interruptions both on the runtime as well as training accuracy and enable users to reach a desired level of accuracy in minimum cost and time. More broadly, this research will democratize machine learning and enable fast and efficient distributed training on unreliable and cheap devices, without requiring access to high-performance computing infrastructure.}

\carlee{other challenges: convergence analysis with changing numbers of workers. it's not clear whether the cost always increases or decreases with runtime and bid prices.}
We have several challenges:

{\bf Random job running time.} Since each a unit price is charged for Spot instance in each time that the instance is running,
to minimize the expected cost, the first question would be that how long should the training job be actually running on such that the job will finally achieves a high quality, \ie, accuracy. The running time is usually known if the workload of the job is per-determined. However, it's unknown for a machine learning training job. Although researchers can set the number of iterations of running the SGD algorithm, the actual wall-clock time can be random. Moreover, the running time of a job performing a distributed SGD is different for different versions, \eg, a synchronous SGD and a batch-synchronous SGD.

{\bf Complication of decision trade-off.} 
Intuitively, if the user increases the bid price, the expected price that is actually charged will be increased, because the expectation of the Spot price that is lower than the bid price (conditioned on the event that the Spot price is lower than the bid price) is increased. Therefore, a user should choose a relatively low bid price in general. However, a low bid price will incur a high probability to be interrupted, and thus a long waiting time. Thus, a user has to make trade-off between a low cost of completing the job and a reasonable completion time, \eg, within the deadline. However, this decision is hard to make when the Spot prices fluctuate in an unknown manner while the job running time is also unknown. 

{\bf Unknown future Spot prices.} Spot prices can change over time. Although Amazon claims that the prices are generally stable and usually only change hourly, it can be volatile in some period of time. As the bid price is a one-time submission without being allowed to re-submit, to minimize the cost, a user has to predict the future Spot price dynamics.

% {\bf Heterogeneous Spot instances.} Although users don't need to choose different types for different workers, they still have to choose one out of multiple options for all workers. Due to various resource configurations, the processing rate can be different, which also determines the running time of the job, given a dataset and the accuracy requirement. Moreover, the Spot price is also different for different types of Spot instances. 


In addressing the above challenges, we make the following contributions. 

\GJ{The contributions listed below are also too detailed. You are trying to give an outline of every section in the paper. Since the system model is not clear yet, we can just put high-level insights/contributions here}

\carlee{Introduce the ways we solve the technical challenges--translate accuracy into iterations, which can then be mapped to job runtimes. Summarize insights (cost non-decreasing with the bid for identical workers, optimal dynamic bidding for non-identical workers.}

%\renewcommand{\labelitemi}{$\rhd$}
%\begin{itemize}
{\em First}, we formulate a stochastic model to characterize the dynamics of the Spot prices and the jobs' running times. We model the Spot price of each type of VM instances into a random variable drawn from an arbitrary i.i.d.~distribution which can be estimated from historical Spot prices. We also assume the running time of each worker to process a given number of data samples (a mini-batch) is drawn from an i.i.d.~distribution. Based on this model, we can simplify the trade-off complication of our decision making, as the unknown dynamics can be estimated before we optimize the bid price. 

{\em Second}, we consider the case where each user adopts identical bid prices for all workers.
We derive a closed-form optimal bid price when the instance type is given, such that the cost is minimized in expectation while the job can be completed within the deadline. We also generalize to optimizing the bid price jointly with choosing the optimal one from multiple types of Spot instances.
For the training algorithm performed by the job, we consider two variants of the synchronous SGD, each of which has a different estimated running time and completion time. We take the exponential and shifted exponential distribution as the examples of the running time per mini-batch distribution, but our proposed bid price optimization method can generalize to other distributions that can be learned beforehand.  

{\em Third}, we then consider non-identical bid prices for different workers within each job. Intuitively, by giving different prices for different workers, the number of active workers will decrease if the price becomes higher, and thus the cost can be possibly decreased. However, fewer active workers lead to a longer running time per iteration. Thus, it is hard to tell whether the total cost can be decreased with some workers having lower bid prices.
By examining the case where the running time per mini-batch follows an exponential distribution, surprisingly we find that the optimal bid prices should be identical for different workers, and we prove this for both variants of the SGD algorithm. 
%For the $N$-batch-synchrounous SGD, the intuitive explanation is that the expected cost per iteration is independent with the number of active workers, and the total expected turns out to be only dependent with the highest bid price among all workers. In the meanwhile, we have to keep the average number of active workers in expectation large enough to satisfy the deadline constraint. Therefore, for any given set of non-identical bid prices $\Vec{b}$, we can decrease the expected cost by changing all bid prices to the one (\ie, the optimal bid price) that yields the same average number of active workers as the $\Vec{b}$. For the $N$-batch-synchronous SGD, 
Further, we examine the shifted exponential distributions and obtain different results from the exponential distribution case. A relatively large difference between the bid prices for different workers can save cost. 

{\em Fourth}, we use data science tools to extract historical Spot prices through Amazon Web Service APIs and adopt the Kernel Density Estimation (KDE) method to fit the spot price into random distributions for predicting the future distributions of the Spot prices. Our trace-driven simulations show that our derived bid prices can save users' cost up to $xx\%$, compared with the bid prices recommended by Amazon Spot market and those randomly predicted.
